Spin-1 Haldane chains of superconductor-semiconductor hybrids

We theoretically explore the possibility of realizing the symmetry-protected topological Haldane phase of spin-1 chains in a tunable hybrid platform of superconducting islands (SIs) and quantum dots (QDs). Inspired by recent findings suggesting that an appropriately tuned QD-SI-QD block may behave as a robust spin-1 unit, we study the behavior of many such units tunnel-coupled into linear chains. Our efficient and fully microscopic modeling of long chains with several tens of units is enabled by the use of the surrogate model solver [Phys. Rev. B 108, L220506 (2023); arXiv:2402.18357]. Our numerical findings indicate that the QD-SI-QD chains exhibit emblematic features of the Haldane phase, such as fractional spin-1/2 edge states and non-vanishing string order parameters, and that these persist over a sizeable region of parameter space.

==> cover.tex <==
Dear Editors,

We hereby submit our manuscript, "Spin-1 Haldane chains of superconductor-semiconductor hybrids", intended as a Regular Article in PRB.

To the best of our knowledge, this is the first work addressing the possibility of realizing the symmetry-protected topological Haldane phase in a superconductor-semiconductor platform, which would certainly broaden the interest in such systems. On a technical side, our thorough numerical simulations show that is has now become possible to construct efficient microscopic models for rather complex quantum-dot-superconductor setups, by the use of our recent methodology based on surrogates models.

Overall, we are confident that our work will appeal to a broad audience of PRB readers, interested in both fundamental and applied condensed matter physics.

Yours sincerely, 
Virgil Baran and Jens Paaske



